SFS: Smart OS Scheduling for Serverless Functions

Serverless computing enables a new way of building and scaling cloud applications by allowing developers to write fine-grained serverless or cloud functions. The execution duration of a cloud function is typically short-ranging from a few milliseconds to hundreds of seconds. However, due to resource contentions caused by public clouds' deep consolidation, the function execution duration may get significantly prolonged and fail to accurately account for the function's true resource usage. We observe that the function duration can be highly unpredictable with huge amplification of more than 50x for an open-source FaaS platform (OpenLambda). Our experiments show that the OS scheduling policy of cloud functions' host server can have a crucial impact on performance. The default Linux scheduler, CFS (Completely Fair Scheduler), being oblivious to workloads, frequently context-switches short functions, causing a turnaround time that is much longer than their service time. We propose SFS (Smart Function Scheduler),which works entirely in the user space and carefully orchestrates existing Linux FIFO and CFS schedulers to approximate Shortest Remaining Time First (SRTF). SFS uses two-level scheduling that seamlessly combines a new FILTER policy with Linux CFS, to trade off increased duration of long functions for significant performance improvement for short functions. We implement {\proj} in the Linux user space and port it to OpenLambda. Evaluation results show that SFS significantly improves short functions' duration with a small impact on relatively longer functions, compared to CFS.

==> _old_related_work_011322.tex <==
\vspace{-8pt}
\section{Related Work}
\label{sec:related}
\vspace{-6pt}

\noindent\textbf{Approximating SRTF.}
Improving turnaround time by approximating SRTF is a well-known approach that has been investigated in many domains~\cite{overload_tit06, mlfq_sigmetrics95, bsd_os_txt, size_sched_tocs03, srtf_mor01}. 
%thus, cloud function scheduling can benefit from decades of research. 
A series of systems use request sizes as the hint to approximate SRTF. 
Size-based scheduling gives preference to requests for small files targeting web servers serving static HTTP requests~\cite{size_sched_tocs03}. 
Similarly, Harchol-Balter~et~al. applied SRTF to webserver request scheduling based on sizes of Linux kernel socket buffers~\cite{srtf_mor01}. 
In principle, 
MLFQ is designed to approximate SRTF. The Solaris 2.6 Time-Sharing scheduler implemented practical MLFQ scheduling by moving jobs across multiple priority levels~\cite{mcdougall2006solaris}. 
Schroeder~et~al. proposed to use MLFQ to alleviate transient overload in web servers~\cite{overload_tit06}. 
%Similar SRTF idea was applied to 
%While cloud function scheduling can benefit from decades of research, {\proj} 
Inspired by these works, {\proj}  presents a practical, approximate SRTF scheduler that addresses many of the challenges in emerging, real-world FaaS workloads. \added{Add Shinjuku etc.}
%presents an approximate SRTF scheduler for emerging, short-function-intensive FaaS workloads
%clearly differentiates against prior work since {\proj} targets emerging FaaS workloads with unique characteristics. 

\noindent\textbf{Serverless Function Scheduling.}
%As FaaS is becoming increasingly popular, FaaS infrastructures and platforms face new scheduling challenges. 
Centralized, core-granular scheduling~\cite{granular_socc19} uses two-level scheduling: it uses centralized scheduling to eliminate queue imbalance and core granular scheduling
%for serverless functions 
to reduce the interference caused by proportional-share.
%time-sharing. 
Core-granular scheduling assumes: 
(1)~non-preemption, meaning a function, once scheduled to a worker core, runs to completion (i.e., running in FIFO),
and (2)~massive-scale, distributed resources, meaning a centralized scheduler can always find available cores to schedule high volumes of function requests.
{\proj} shares similar goals but targets highly consolidated function environments, where a single FaaS server 
may be over-committed with a request arrival rate higher than the service rate. 
%serves many more function requests in a unit of time than the cores this server has and FIFO causes high queuing delay %{\bf rephrase?}. 
%FnSched~\cite{fnsched_wosc19}, Nightcore~\cite{} 
Another line of work is focused on distributed or FaaS platform-level function scheduling~\cite{fnsched_wosc19, nightcore_asplos21, olsched_minmove18} by using function placement optimization, low-latency I/Os, and data locality. 
Serverless dataflow frameworks use variants of cluster scheduling techniques~\cite{caerus_nsdi21, wukong_socc20, pywren_socc17, numpywren_socc20, sequoia_socc20} for serverless workflow applications. These works use the Linux scheduler for ``last mile'', OS-level task scheduling and would benefit from {\proj}.

\noindent\textbf{User-Space Threading.}
A large body of works is focused on enabling efficient user-space threading. Examples include Arachne~\cite{arachne_osdi18}, $\mu$Thread~\cite{muthread}, libinger~\cite{libinger_atc20}, Go's runtime scheduler~\cite{go_scheduler}, and more. Compared to these user-space threading libraries, {\proj} is more lightweight. Unlike these solutions, {\proj} seamlessly combines a custom, user-space scheduler with CFS to construct a unified scheduling framework for serverless function scheduling. 


\if 0
%\noindent\textbf{Low-Latency I/O Scheduling.}
\noindent\textbf{Scheduling for Fine-Grained I/O Tasks.}
%A large body of research aims for achieving microsecond-scale I/Os.
%via new scheduling approaches. 
Systems such as Arrakis~\cite{arrakis_osdi14}, IX~\cite{ix_osdi14}, and MICA~\cite{mica_nsdi15} bypass the kernel with a shared-nothing architecture, which allows I/O requests to run to completion without the need to be rescheduled. 
%Systems such as 
Shenango~\cite{shenango_nsdi19}, Shinjuku~\cite{shinjuku_nsdi19}, and ZygOS~\cite{prekas2017zygos} use scheduling techniques such as core re-allocation, preemption, and work-stealing for improved tail latency for network I/O-intensive applications. 
%Arachne~\cite{arachne_osdi18} and PerfIso~\cite{perfiso_atc18} uses dynamically-allocated, designated cores to minimize interference. 
%These techniques such as low-latency network I/O scheduling
Undoubtedly, these techniques can be used to improve the scalability and performance of function request dispatching, which is one level above {\proj}. 
\fi 





==> cloud_measurement_bakcup.tex <==

\begin{table}[t]%{0.26\textwidth}
%\vspace{-20pt}
%\vspace{10pt}
\caption{
%Diverse characteristics of the studied FaaS applications. 
The {\bf max/min ratio} (the ratio of the maximum duration and the average 
of the minimal duration) of studied functions.
%FaaS applications. 
%Functions were configured with 256~MB memory.
%\added{Memory sizes?}
%The ideal execution duration is calculated by averaging the minimum duration of all sampled intervals.
}
\vspace{-15pt}
\begin{center}
\scalebox{0.87}{
\begin{tabular}{lrrrrrr}
%\hline
%{}          & \multicolumn{3}{c}{\bf Max/min ratio}  & {}   & {} \\
{\bf Func.} & {\bf AWS} & {\bf GCF} & {\bf ACF} & {\bf CPU-intensive}  & {\bf I/O-intensive}   \\ 
\Xhline{2\arrayrulewidth}
{\fib}     & {$6\times$}  & {$10\times$}  & {$2029\times$}    & {\cmark}  & {\xmark}    \\
{\mg}      & {$6\times$}  & {$7\times$}   & {$2014\times$}     & {\xmark}  & {\cmark}    \\
{\sa}      & {$18\times$} & {$405\times$} & {$2204\times$}  & {\cmark}  & {\cmark}    
%\hline
\end{tabular}
}
%\vspace{-5pt}
\label{tbl:func}
\vspace{-15pt}
\end{center}
\end{table}






\vspace{-4pt}

\begin{figure*}[t]
\vspace{-15pt}
\begin{center}
\subfigure[{\fib} (AWS).] {
\includegraphics[width=.31\textwidth]{figs/moti/aws_fib.eps}
\label{fig:aws_fib}
}
\hspace{-9pt}
%\vspace{-20pt}
\subfigure[{\mg} (AWS).] {
\includegraphics[width=.31\textwidth]{figs/moti/aws_md.eps}
\label{fig:aws_md}
}
\hspace{-9pt}
\subfigure[{\sa} (AWS).] {
\includegraphics[width=.31\textwidth]{figs/moti/aws_sa.eps}
\label{fig:aws_sa}
}
%\vspace{-20pt}
\subfigure[{\fib} (GCF).] {
\includegraphics[width=.31\textwidth]{figs/moti/gcf_fib.eps}
\label{fig:gcf_fib}
}
\hspace{-9pt}
\subfigure[{\mg} (GCF).] {
\includegraphics[width=.31\textwidth]{figs/moti/gcf_md.eps}
\label{fig:gcf_md}
}
\hspace{-9pt}
\subfigure[{\sa} (GCF).] {
\includegraphics[width=.31\textwidth]{figs/moti/gcf_sa.eps}
\label{fig:gcf_sa}
}
%\vspace{-20pt}
\subfigure[{\fib} (ACF).] {
\includegraphics[width=.31\textwidth]{figs/moti/azure_fib.eps}
\label{fig:azure_fib}
}
\hspace{-9pt}
\subfigure[{\mg} (ACF).] {
\includegraphics[width=.31\textwidth]{figs/moti/azure_md.eps}
\label{fig:azure_md}
}
\hspace{-9pt}
\subfigure[{\sa} (ACF).] {
\includegraphics[width=.31\textwidth]{figs/moti/azure_sa.eps}
\label{fig:azure_sa}
}
\vspace{-10pt}
\caption{Timeline of function duration in three providers. 
AWS: AWS Lambda; 
GCF: Google Cloud Functions;
ACF: Azure Cloud Functions. 
%\yuec{Yuqi TODO: X tics change to 1 - 14, with a label ``Day''}
}
\label{fig:moti_cloud_study}
\end{center}
\vspace{-10pt}
\end{figure*}

\subsection{Public Cloud Measurement}
\label{subsec:moti_public_cloud}
%\vspace{-4pt}

%Next, we performed a week-long measurement study over three different function applications, 
Next, we conducted a two-week-long (August 29 - September 12, 2021) measurement study to empirically quantify the duration amplification of cloud functions from three major FaaS providers, AWS, Google, and Azure. We selected three representative function applications~\cite{serverless_arch_micro19,python_bench}, which exhibit diverse CPU and I/O characteristics, as listed in Table~\ref{tbl:func}.  
\textbf{Fibonacci sequence} ({\fib}) calculates a sequence of $N$ Fibonacci numbers and is CPU-heavy. In our experiment, we chose three $N$s: 20, 25, and 30, but often only report the results of 25 as those of 20 and 30 showed similar trends. 
\textbf{Markdown generation} ({\mg}) reads a JSON file from the function's local storage and transfers it to the markdown format; {\mg}'s execution is I/O-intensive. 
\textbf{Sentiment analysis} ({\sa}) reads a file that contains a sentiment vocabulary dictionary and then predicts the sentimentality given a target sentence; {\sa} is both CPU-intensive and I/O-intensive.  
%In this experiment 
We tested functions with 256-5120~MB memory, but due to space constraint we only report results for functions with 256~MB.

%\emph{markdown generation} ({\mg}), and \emph{sentiment analysis} ({\sa}), %with various CPU and memory configurations. with various CPU and I/O patterns. Table~\ref{tbl:func} 

In the experiment, we invoked each function with the same code every three seconds for a period of two weeks. We intentionally excluded invocations that triggered a cold start. 
%from August 30 to September 12, 2021. 
Figure~\ref{fig:moti_cloud_study} reports the execution duration percentile breakdown of each 30-minute interval. 
We make the following observations.
(1) The function execution duration exhibits surprisingly high variation on all three FaaS platforms; for example, the maximum duration was up to  $405\times$ higher than the minimum duration for GCF, as shown in Table~\ref{tbl:func} and Figure~\ref{fig:gcf_fib}-\ref{fig:gcf_sa}. 
(2) Interestingly, the minimum duration results are very stable for all functions on all FaaS platforms: our hypothesis is that the stable minimum results may be due to temporary, lesser, multi-tenant contention, thus representing a best-case (i.e., ideal) performance that a user would desire to achieve. 
%{\bf More importantly, this sets the target performance that one would like to achieve ideally.}
(3) ACF shows completely different spiky patterns than AWS and GCF; this is possible because ACF allows multiple concurrent invocations of the same function in parallel within the same function environment~\cite{azure_parallel_inv};
furthermore, the duration breakdown patterns shown in Figure~\ref{fig:azure_fib}-\ref{fig:azure_sa} are consistent with what was reported in \cite{serverless_in_the_wild}.
%\yuec{TODO: further observations due to pending {\mg} and {\sa} results.}

\vspace{-4pt}
\paragraph{Implication 2:}
\emph{Alleviating the high amplification of function executions may reduce the overcharges and improve the fairness for FaaS users.}








%%%%%%%%%%%%% overload
\begin{figure}
\begin{center}
\subfigure[Timeline of queuing delays.] {
\includegraphics[width=.23\textwidth]{figs/switch_delay.eps}
\label{fig:delay}
}
\hspace{-12pt}
\subfigure[CDF of function duration.] {
\includegraphics[width=.23\textwidth]{figs/switch_exec.eps}
\label{fig:switch_cdf}
}
\vspace{-14pt}
\caption{Handling transient overload.}
\label{fig:switch}
\end{center}
\vspace{-15pt}
\end{figure}

%%%%%%%%%%%%%% OL
\begin{figure*}[t]
%\vspace{-12pt}
\begin{minipage}{\textwidth}

\begin{comment}
\begin{minipage}[b]{0.33\textwidth}
%\begin{table}[t]%{0.26\textwidth}
%\vspace{-20pt}
%\vspace{10pt}
\vspace{-15pt}
\begin{center}
\scalebox{0.87}{
\begin{tabular}{lrrrrrr}
%\hline
%{}          & \multicolumn{3}{c}{\bf Max/min ratio}  & {}   & {} \\
{\bf Func.} & {\bf CPU-intensive}  & {\bf I/O-intensive}   \\ 
\Xhline{2\arrayrulewidth}
{\fib}      & {\cmark}  & {\xmark}    \\
{\mg}       & {\xmark}  & {\cmark}    \\
{\sa}       & {\cmark}  & {\cmark}    
%\hline
\end{tabular}
}
\caption{
%Diverse characteristics of the studied FaaS applications. 
The {\bf max/min ratio} (the ratio of the maximum duration and the average 
of the minimal duration) of studied functions.
%FaaS applications. 
%Functions were configured with 256~MB memory.
%\added{Memory sizes?}
%The ideal execution duration is calculated by averaging the minimum duration of all sampled intervals.
}
%\vspace{-5pt}
\label{tbl:func}
\vspace{-15pt}
\end{center}
%\end{table}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%\hspace{-1em}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}

\begin{minipage}[b]{0.4\textwidth}
\begin{center}
% \includegraphics[width=1\textwidth]{plots/latency-zoomin.pdf}
\includegraphics[width=1\textwidth]{figs/openlambda/vary_cfs.eps}
\end{center}
\vspace{-10pt}
\caption{
Function duration CDF.
}
\label{fig:ol_cdf}
\end{minipage}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%\hspace{-1em}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.4\textwidth}
\begin{center}
% \includegraphics[width=1\textwidth]{plots/latency-zoomin.pdf}
\includegraphics[width=1\textwidth]{figs/openlambda/ctx_diff.eps}
\end{center}
\vspace{-10pt}
\caption{
Logarithm of context switch ratio.
}
\label{fig:ol_ctx_diff}
\end{minipage}

\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hfill
%\hspace{-1em}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}[b]{0.33\textwidth}
\begin{center}
\includegraphics[width=1\textwidth]{figs/openlambda/ctx_cdf.eps}
\end{center}
\vspace{-10pt}
\caption{
Context switch CDF. 
% \yuec{\# VM -> Tree height}
}
\label{fig:ol_ctx_cdf}
\end{minipage}
\end{comment}

\end{minipage}
\vspace{-10pt}
\end{figure*}
